Motion Prediction Under Multimodality with Conditional Stochastic Networks

Given a visual history, multiple future outcomes for a video scene are equally probable, in other words, the distribution of future outcomes has multiple modes. Multimodality is notoriously hard to handle by standard regressors or classifiers: the former regress to the mean and the latter discretize a continuous high dimensional output space. In this work, we present stochastic neural network architectures that handle such multimodality through stochasticity: future trajectories of objects, body joints or frames are represented as deep, non-linear transformations of random (as opposed to deterministic) variables. Such random variables are sampled from simple Gaussian distributions whose means and variances are parametrized by the output of convolutional encoders over the visual history. We introduce novel convolutional architectures for predicting future body joint trajectories that outperform fully connected alternatives \cite{DBLP:journals/corr/WalkerDGH16}. We introduce stochastic spatial transformers through optical flow warping for predicting future frames, which outperform their deterministic equivalents \cite{DBLP:journals/corr/PatrauceanHC15}. Training stochastic networks involves an intractable marginalization over stochastic variables. We compare various training schemes that handle such marginalization through a) straightforward sampling from the prior, b) conditional variational autoencoders \cite{NIPS2015_5775,DBLP:journals/corr/WalkerDGH16}, and, c) a proposed K-best-sample loss that penalizes the best prediction under a fixed "prediction budget". We show experimental results on object trajectory prediction, human body joint trajectory prediction and video prediction under varying future uncertainty, validating quantitatively and qualitatively our architectural choices and training schemes.

==> MotionPrediction (4)/abstract_arxiv.tex <==

\begin{abstract}
Given a visual history,  
multiple  future  outcomes for a video scene are  equally probable, in other words,  
the distribution of future outcomes has multiple modes.  Multimodality is notoriously hard to handle by standard regressors or classifiers: the former regress to the mean and the latter discretize a continuous high dimensional output space.  
In this work, we present  stochastic neural network architectures 
that handle such multimodality through stochasticity: future  trajectories of objects, body joints or frames are  represented as deep,  non-linear transformations of  random (as opposed to deterministic) variables. 
Such random variables are sampled from simple Gaussian distributions whose means and variances are parametrized by the output of  convolutional encoders over the visual  history. We introduce novel convolutional   architectures for predicting future body  joint trajectories that outperform fully connected alternatives \cite{DBLP:journals/corr/WalkerDGH16}. We 
introduce stochastic spatial transformers through optical flow warping for predicting  future frames, which outperform  their deterministic equivalents  \cite{DBLP:journals/corr/PatrauceanHC15}.  
Training  stochastic networks involves an  intractable marginalization over stochastic variables. We compare various training schemes that handle such marginalization through a) straightforward sampling from the prior, b) conditional variational autoencoders  \cite{NIPS2015_5775,DBLP:journals/corr/WalkerDGH16},  and, c) a proposed K-best-sample loss that penalizes the best prediction  under a fixed  `` prediction budget". We show  experimental results on object trajectory prediction, human body joint trajectory prediction and video prediction under  varying future uncertainty, validating quantitatively and qualitatively our architectural choices and training schemes. 
\end{abstract}



==> MotionPrediction (4)/conclusion_arxiv.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented stochastic neural networks for multimodal motion forecasting for object, body joint and frame predictions. We presented architectural innovations as well as novel training schemes and extensive evaluations of those in various benchmarks. Our work aims to help understanding stochastic networks and their applicability for forecasting, and the difficulties (or not) of their training, building upon and extending recent previous works.   
We discussed both object and body joint trajectory prediction that uses human annotations for future outcomes as well as self-supervised video prediction that uses the next frame as ground-truth. The longer the temporal horizon for the prediction, and the shorter the temporal history to condition upon, the larger the uncertainty and the larger the benefit from incorporating stochasticity.  
%Motion forecasting is of central importance for robotics, autonomous navigation and augmented reality, and we expect our model to find use in those domains.  
Our model offers a simple solution to  multimodal prediction of large continuous spaces and we expect it will  be useful in  domains with uncertainty beyond motion prediction. 

==> MotionPrediction (4)/experiments_arxiv.tex <==


\begin{figure}%[h!]
\centering
\includegraphics[width=0.99\linewidth]{figs/newfigs/dronefig.pdf} 
\caption{\textbf{Object motion trajectory  prediction} in the drone Stanford dataset of \cite{DBLP:journals/corr/RobicquetASADWS16}.   A single frame is used as input ($\Nf=1$).  This is a case of \textit{extreme uncertainty}:  we do not have any idea regarding the direction of object's motion.  The first column shows the overhead scene and the input visual glimpse and second column shows the groundtruth trajectory. Dark blue denotes high sample density and light blue denotes low sample density.  MCbest predicts more diverse outcomes (e.g., row 3) in comparison to the rest.  
}
\label{fig:alahiqual}
\end{figure}

\begin{figure*}%[t!]
\centering
 \includegraphics[width=1.0\linewidth]{figs/newfigs/drone.pdf} 
\caption{
\textbf{Object trajectory prediction} in the Drone Stanford  dataset~\cite{DBLP:journals/corr/RobicquetASADWS16} under varying number of  input frames $\Nf$.  We show top$k$ error,  for $k=1$ and $k=4$ . \textit{Col 1:} Forecasting future motion trajectory from a single frame.  This is a case of extreme uncertainty and MCbest outperforms the rest on top-4 error. %, since explicitly, during training, optimizes a 15-best loss. 
%\textit{Col 4:} 
When a long visual history is used as input ($\Nf=8$), the benefit of stochastic models  over a  deterministic regression baseline is smaller, as uncertainty in prediction decreases (column 4). 
%Yet, they are important to predict accurately (e.g., at intersections) and this justifies the use of rich predictive models that handle multimodality.
%. Note though that 
%in our dataset, in most of the cases a linear motion model  would suffice. 
%it is \textit{at the intersections that a multimodal predictive model is needed}, and this is precisely when good predictions are crucial, e.g., to adapt a self-driving car's behavior based on anticipated pedestrian motion. 
%at those points in tiem that a good predictive model is necessary.
%\textit{Row~1:} Top~1  trajectory prediction error.  \textit{Row 2:} Top~4 trajectory prediction error. \textit{Cols 1,3:} Only the current frame is provided as input. \textit{Cols 2,4:} A concatenation of the three most recent frames is provided as input. MCmin though having worse top-1 error has the best top-4 error, since explicitly, during training, optimizes a K-best loss. Regression does not generalize well, as expected. MClogsumexp has a much longer training time till convergence in this experiment.
}
\label{fig:dronecurves}
\end{figure*}

\begin{figure}
\centering
 \includegraphics[width=1.0 \linewidth]{figs/fcconv1.pdf} 
\caption{ \textbf{Body joint trajectory forecasting} in the H3.6M test set. All actions categories are considered and five frames are used as input ($\Nf=5$). All models apart from \textit{regressionFC} share the same architecture that use  conv-indexed decoders. The regression baseline \textit{regressionFC} has a fully-connected decoder instead for comparison.  \textbf{Fully connected decoders  under-fit our dataset and failed to minimize the error}. For clarity we show only the fully connected regression model since the stochastic fully connected models exhibit similar behavior.  Conditional variational autoencoders outperform all other training schemes in this experiment.  }
\label{fig:fcconvcurves1}
\end{figure}


\begin{figure}
\centering
 \includegraphics[width=1.0 \linewidth]{figs/fcconv2.pdf} 
\caption{ \textbf{Video prediction} in the H3.6M test set from a single image ($N=1$). \textit{(a)} We compare $15$-best-loss (\textit{MCbest})  against conditional variational approximations (\textit{VA}). $15$-best-loss has higher top1 error than VA but lower top4 and top14 error. \textit{(b)} $K$-best loss under varying $K$: as we increase number of samples $K$, top1 error gets worse and top4 decreases, as expected. $K$ is a hyper-parameters and depends on the amount of anticipated uncertainty.}
\label{fig:fcconvcurves2}
\end{figure}



\begin{figure*}%[t!]
\centering
 \includegraphics[width=1.0\linewidth]{figs/newfigs/videoprediction.pdf} 
\caption{ \textbf{Video prediction} results in MoSeg and H3.6M datasets. %conditioning on one and two frames. 
%We only trained 5-best-loss in MoSeg due to GPU memory requirements. In H3.6M,  the image crop is smaller (64X64), thus we managed to train 15-best-loss. 
}
\label{fig:videopredictcurves}
\end{figure*}


%\newcommand*{\TitleParbox}[1]{\parbox[c]{1.75cm}{\raggedright #1}}%







\section{Experiments}

We test the performance of our stochastic network models in three tasks: (a) forecasting future motion of human body joints, (b) forecasting video frames, and (c) forecasting future object motion from overhead cameras, and compare against losses and architectures considered in previous works. 
We  compare the following training schemes presented in Section \ref{sec:model}: (a)  a sample approximation to the marginal likelihood (\textit{MCML}), (b) $K$-best-sample loss (\textit{MCbest}), (c) conditional variational autoencoder (\textit{VA}) for the various architectures we consider in each task. We also consider   a regression model (\textit{regression}) that has similar architecture to the stochastic alternatives in each experiment  but that does not have any stochastic units and  minimizes a regression loss. 

\paragraph{Evaluation metric} We  quantify how well our models perform on predicting the distribution of the future outcomes in our datasets, let it be object trajectories, body joint trajectories or future frames, using top$k$ error, $k \in 1 \cdots 15$: top$k$ error measures the lowest of the errors (against ground-truth) among the top $k$ predictions, where predictions are ordered according to model's confidence. For our stochastic networks, we obtain multiple predictions by sampling  $\zz$  (without ensuring diversity) and decoding it to $\hat{yout}$  and ordering the predictions according to the $\zz$ probability  (in decreasing order) while keeping the top $k$ most confident. Top$k$ error is a meaningful measure in case of uncertainty, when there is no one single best solution, and has been employed widely, e.g.,  in the Imagenet Image classification task \cite{deng2009imagenet}, which has potentially much less uncertainty than our forecasting setup. For regression models, we only have one prediction available and thus all top$k$ errors are identical.

%Top$k$ error metric considers the best proposal from a budget of $K$ predictions,  a meaningful measure in case of uncertainty. In VA, MC-ML and MC-best, output trajectory samples are obtained by sampling from the $\zz$ Gaussian distributions without ensuring diversity.
%Multiple possible outcomes are plausible in each example, dependening on the degree of uncertainty: e.g., given a \textbf{single} image from an overhead camera, the centered object may move in many different directions. Such uncertainty decreases as we increase the length of the conditioning visual history ($\Nf$). To measure such agreement we use top-$k$ error, $k \in 1 \cdots 15$.


%Given the multimodality of the domain (pedestrians, bicyclists, buses etc can all take multiple possible future paths) we use top-$k$ error to evaluate all methods: a prediction is assumed correct if it lies within the top $k$ predictions, where predictions are ordered according to model's confidence.
% We use top-$K, K \in 1 \cdots 15$ error metrics,  which consider the best proposal from a budget of $K$ predictions,  a meaningful measure in case of uncertainty. In VA, MC-ML and MC-best, output trajectory samples are obtained by sampling from the $\zz$ Gaussian distributions without ensuring diversity.
 
 
%, similar to \cite{fragkiadaki2015learning,DBLP:journals/corr/FragkiadakiLM15} for object trajectory prediction or work of \cite{DBLP:journals/corr/PatrauceanHC15} for frame prediction.  We also compare against a model with fully connected decoder trained with variational autoencoder similarly to \cite{} for dense frame prediction from static images.



\begin{figure*}%[h!]
\centering
\includegraphics[width=0.99\linewidth]{figs/newfigs/videopredfig.pdf} 
\caption{\textbf{Video prediction} in MoSeg (first five columns) and H3.6M (last five columns) using $Nf=2$ frames as input. \textit{Top row:} last frame of visual history. \textit{Bottom Row:} predicted flow field. \textit{Middle Row:} predicted frame by warping. The forecasted flow fields correctly delineate the moving objects. The visual realism of the predicted frames is a benefit of using motion driven differentiable warping  \cite{DBLP:journals/corr/ZhouTSME16}   as opposed to direct pixel  generation through standard deconvolution networks.} 
\label{fig:videopredres}
\end{figure*}






\paragraph{Human body joint trajectory forecasting}
We use the Human3.6M (H3.6M) dataset of Ionescu et al. \cite{h36m_pami}. H3.6M contains videos of actors performing activities and provides annotations of body joint locations at every frame, recorded from a Vicon system. We split the videos according to the human subjects, having subject with id=5 as our test subject. 
%We consider videos of the walking activity. 
We consider videos of all activities. We center our input glimpses around the human actor by using the bounding box provided by the dataset on the latest history frame and crop all history images with the same box (so that only the human moves and the background remains static, as is the case also in the original frame). 
 For training, we pretrained the encoder for body joint detection in the same dataset, and then finetuned the whole model in the forecasting. We consider two types of decoder subnetworks: a four layer fully connected decoder considered in \cite{DBLP:journals/corr/WalkerDGH16} and a conv-indexed decoder, described in Section \ref{sec:model}. % that is fully convolutional, uses skiplayers and predicts joint trajectories with one linear layer per joint using features indexed from the corresponding current joint locations.  


Our evaluation criterion is L2 distance between predicted and ground-truth instantaneous velocities of all body joints, averaged over the time horizon of the prediction. We use $\Hor=15$.  
We show quantitative results in Figure \ref{fig:fcconvcurves1} (a) for $\Nf=5$ frames in the visual history input to the model. All models with fully connected decoders failed to minimize the error in our experiments and  under-fit the training set. We show in the figure only the regression baseline for clarity (\textit{regressionFC}), as the other curves are identical. Models with  conv-indexed decoders fit the data effectively, and the VA training scheme performed the best.  For extensive qualitative results please see our   \href{https://sites.google.com/site/conditionalstochasticnets/}{online website}.

Conv-indexed decoders assume we know the pixel coordinates $(x,y)$ of the joints whose trajectories we want to predict in the latest frame of the visual history. Such knowledge  is indeed available, without which prediction of velocities (accumulated in time to form predicted $(x,y)$ locations) would not be meaningful.  We note that fully connected decoders effectively worked for the much easier, close to deterministic, problem of  predicting body joint trajectories \textit{only for the Walking activity} which suggests that architectural considerations are important as the forecasting problem becomes harder and more diverse. 
%We include Walking only results in the supplementary material \href{https://sites.google.com/site/conditionalstochasticnets/}{online website}

%For dense trajectory prediction considered in previous works \cite{} since the num
%The overshooting of top-1 error of MCmin in this case is because the number of samples $\nsamples=15$ is large compared to the low uncertainty of the walking activity. As shown in Figure \ref{fig:H36} rightmost column, the errors for MC-best converge fast after  4 sampled proposals, which means the correct solution is always contained within the top 3-4 proposals. Please see video results in our supplementary material.
%So, MC-best comes with the size of prediction budget as a parameter



\paragraph{Video prediction}
We use  the Freiburg-Berkeley Motion Segmentation (MoSeg) dataset  of  \cite{springerlink:10.1007/978-3-642-15555-0_21} and  the Human3.6M (H3.6M) dataset of  \cite{h36m_pami}. MoSeg  contains high resolution videos of people, animals, vehicles and other moving objects; the camera  may be moving or static and the frame rate varies from video to video. H3.6M contains videos of a static camera and constant frame rate.  
We applied frame-centric video prediction in MoSeg and object-centric prediction in H3.6M (same as above, but this time we predict the whole frame rather than body joint trajectories). 
 In this way, we can test video prediction both in controlled and ``in-the-wild'' setups. In MoSeg, we follow the official train and test split of the dataset and train our video prediction models from scratch. In H3.6M, we use the same split as for body joint prediction. The input to the network is 128 X 320 for MoSeg and 64X64 for H3.6M. 
 MCML has shown the worst performance so far and since for frame prediction each sample is a whole decoded frame rather than a small set of trajectories we did not consider MCML for this experiment. 
%We instead focus on MCbest and VA.  
%Using fully convolutional decoders with skip connections, as those used by our \ESD for video frame prediction, would not allow limited GPU-memory to test sampling based approaches, that is our MC-best and MC-ML models. 
Due to GPU memory limitations, we could only test 5-best-loss for MoSeg while for H3.6M we test 15-best-loss (since the input to the network is smaller).  
We also compare against a regression baseline that predicts a single flow field and warps to generate the future frame, similar to the model of  \cite{DBLP:journals/corr/PatrauceanHC15}.  
%further compare a  regression non-stochastic model with an \ESD model trained using the variational autoencoder (VAE). We evaluate both fully convolutional stochastic layers and fully connected layers. 
%In the absence of an appropriate quantitative evaluation measure, we  use pixel matching error, that is, average pixel L2 loss between next ground-truth frame and predicted frame.  

Quantitative results showing the L2 loss between next ground-truth frame and predicted frame for the test set of the two datasets are shown in Figures \ref{fig:videopredictcurves}, \ref{fig:fcconvcurves2} and qualitative results are in Figure~\ref{fig:videopredres}. 
All models fail to minimize the prediction error in MoSeg dataset when only one frame is considered due to camera motion: camera motion dictates the appearance of the next frame and is impossible to be predicted from a single frame. This is one reason previous works use  background subtraction to stabilize the video \cite{DBLP:journals/corr/WalkerDGH16,vondrick2016generating}. On the contrary, in H3.6M  the camera is not moving and a single frame  suffices to make plausible predictions of future flow fields. 
%For qualitative results of diverse next frame prediction, please see our  \href{https://sites.google.com/site/conditionalstochasticnets/}{online website}.
Video results and diverse samples for future frames are available at our \href{https://sites.google.com/site/conditionalstochasticnets/}{online website}  as gifs,  since they are often too subtle to see in a static image.

%We show average pixel L2 loss between best framne and predicted frame. 
%The non-convolutional stochastic layers outperform convolutional ones, which suggests that potentially a sequential in space sampling of the stochastic codes across the grid may be an easier way for the decoder to consolidate the different modes in different parts of the image. 
%Incorporating stochasticity is beneficial under high uncertainty ($\Nf=1$) , particularly in this scenario that prediction concerns very short term horizons instead of long temporal horizon on motion trajectory forecasting experiments.




\paragraph{Object future motion trajectory prediction}
We use the Stanford Drone dataset introduced in Robicquet et al. \cite{DBLP:journals/corr/RobicquetASADWS16}, the largest overhead dataset that has been collected so far, with a drone flying above various locations in the Stanford campus. Trajectories of vehicles, pedestrians, bikers, bicyclists, skateboarders etc, as well as their category labels have been annotated. We split trajectories into train and test set randomly.  We use a short sequence of $\Nf$ square visual glimpses around the target of interest (again following the principle of object-centric prediction) as input to our model and predict future motion for the subsequent $\Hor=100$ frames.   We do not use the annotated category labels. We randomly split object trajectories into train and test sets. 
Our evaluation criterion is L2 distance between predicted and ground-truth instantaneous velocities, averaged over the time horizon of the prediction.

We show quantitative results of our models and a regression baseline in Figure \ref{fig:dronecurves}. The deterministic regression baseline is similar to the model used in \cite{fragkiadaki2015learning} for predicting trajectories of Billiard balls in simulated (deterministic)  worlds. Under uncertainty,  regression  has higher top1  error than VA, and  much higher error than top4 errors of VA and $15$-best-loss, for any number of input history frames $\Nf$ (for $\Nf=1$, VA takes much longer to train than regression). 

\textbf{As the length of the history increases, uncertainty decreases} and regression  becomes more competitive. 
%Indeed, regression is not outperformed by the stochastic alternatives by a large margin for $\Nf>1$ . 
Indeed, most of the times a linear object motion model suffices. It is at the \textit{intersections} that a multimodal predictive model is needed, but these are precisely the cases when good predictions are crucial, e.g., to adapt a self-driving car's behavior based on anticipated pedestrian motion.  
%Regression  has the smallest \textit{training} error but fails to generalize as well as the stochastic models. 
Please see our \href{https://sites.google.com/site/conditionalstochasticnets/}{online website} for video results.



%We show quantitative results of our model and baselines in Figure \ref{fig:alahiqual}. When only one frame is used as input ($\Nf=1$) the uncertainty is higher and both top-1 and top-4 errors are higher.   For top-1 error, VAE outperforms MCmin since MCmin has been trained to produce the best outcome under 15 samples, rather than 1, so this is expected.  MCmin    shows the largest diversity among all methods having the lowest  top-4 error. The regression baseline does not have more than 1 proposal to output; though it overfits very well in the training set, it  generalizes  poorly.  MClogsumexp shows a sharp error decrease after 2 million iterations. Though it does better than regression, it exhibits limited diversity, as its top-4  error is not much lower than the top-1 error.  
%The longer training times are attributed to small batch sizes. 
%In this case, we believe the longer training time is due to the 
%We conclude that Monte Carlo sampling for diverse prediction under maximum likelihood is not a suitable loss.

%Qualitative results in Figure \ref{fig:alahiqual} validate our findings; the distribution of samples from MCmin is far more diverse in comparison to the other models. For  detailed curves obtained by 
%continuously varying the number of samples, please see our supplementary material.






\subsection{Implementation details.} \label{sec:details}
Our encoder $\encoder$ is a convolutional network variant of the Inception architecture~\cite{szegedy2015going}. We pre-train our encoders on the ImageNet classification task by replicating the weights of the first convolutional layer as many times as the number of frames in the input glimpse volume. For body joint trajectory forecasting, we pretrain our encoder on body joint classification in H3.6M dataset. 
%The input to our network is 128X128 for all tasks apart from video prediction in the MoSeg dataset where it is 256X256. 
We use skip layers in the tasks of body joint trajectory forecasting and video forecasting.
%Its input is a sequence of $\NN$ visual glimpses centered around the object of interest warped 
%In the case of object-centric visual glimpses, the visual input is warped to spatial size of $299 \times 299$, else we use the frame size.  %The glimpse size is kept large enough to capture the relevant spatial context for prediction. 
%(we use $600 \times 600$ resolution frames from which we 
%create $299\times 299$ glimpses in experiments).
%a sequence of visual glimpses --- square image crops --- centered around the moving object of interest (see Figure~\ref{fig:model} for an illustration). 
%We use fully connected decoders for object and body-joint prediction and fully convolutional decoders with skip layers from encoder feature layers for video prediction. 
%We use a 5-layer fully connected decoder for object trajectory forecasting,   and a 6-layer fully convolutional decoder for optical flow and video frame prediction. 
The stochastic variables are replicated across the width and height of the top encoder layer in case of fully convolutional decoders. 
%We considered both fully convolutional and fully connected stochastic layers. In case of fully convolutional stochastic layers, we have a spatial grid volume of means and variances, each controlling the distribution of the stochastic codes around that spatial location. Similarly, means and variances are convolutionally computed. The codes are sampled independently across the spatial grid, in which case it is the decoder's responsibility to consolidate the different modes. Conditional spatial sampling of the codes should by beneficial but was not considered in this work.
%and our sampled  stochastic codes similarly form a spatial grid volume of the same size.
%During training, for each example, we draw $\nsamples =15$ sampled vectors/ volumes. 
We represent output motion trajectories with a sequence of instantaneous velocities $\tr=\{(\Delta{\trx_t}, \Delta{\try_t}), \ t=0,\dots,\Hor\}$, where $\Hor$ is a prediction horizon. 
We conduct our training and evaluation using TensorFlow~\cite{citeulike:13838961}, a publicly available deep learning package. 
%For more implementation details, please refer to our supplementary material due to lack of space.



==> MotionPrediction (4)/introduction_arxiv.tex <==
\section{Introduction}
\label{sec:introduction}

%\TODO{RS - Made small edits starting from abstract and left TODOs like this when I wasn't sure.}

%In dynamic environments, 
%Predicting the motion of people and objects is necessary to direct gaze, avoid collisions and enable effective interactions with a dynamic world in a timely manner, while anticipating for the lag inherent in mechanical systems. In infants, the ability for such predictive tracking, a.k.a.\ smooth pursuit~\cite{Hofsten19971799}, quickly reaches adult performance in the first months after birth.  The development of expectations over future outcomes is ubiquitous in our interaction with the world: while watching a scene, we are perfectly at ease with one of  its many possible future evolutions, e.g., students in class are expected to take notes, raise hands to ask or answer questions, or stare at their laptops,  but we do get very surprised under unexpected outcomes, e.g., if a student raises her hand horizontally instead of upwards, or looks backward instead of forward during a lecture. How do we get to develop such expectations over \emph{diverse} future behaviours? 
Humans live in the future: we constantly predict what we are about to perceive (see, hear or feel)  during our interactions with the world, and learn from the deviations of our expectations from the reality \cite{de-Wit8702}. % believe prediction is viable for 
%Humans constantly predict what they are about to see during their interactions with the world: 
While watching a scene, we are perfectly happy with one of its \textit{many} possible future evolutions, 
%e.g., students in class are expected to take notes, raise hands (to ask/answer questions, or stare at their laptops,  
but unexpected outcomes cause surprise.  Predictive computational models should  similarly be able to \textit{predict any of the  different modes of the  distribution of future outcomes}. 


%In this work, we study object motion trajectories, body joint trajectories or whole frames as representations of the future outcomes which we want to predict.
%outcomes. 





%In Computer Vision, previous works of \cite{} sample unconditional Gaussian noise and concatenate it to the network input, and decode it to video frames in \cite{} and dense point trajectories in \cite{}. 
We  present stochastic neural network architectures that predict samples of  future outcomes conditioned on a history of visual glimpses, and apply them to the tasks of object trajectory, body joint trajectory  and  frame forecasting (Figure \ref{fig:Pnets}).  
%Stochastic neural networks have been recently proposed as a viable alternative 
%to deterministic networks for handling multimodality of the output space \cite{DBLP:journals/corr/WalkerDGH16,NIPS2016_6552}. 
%and have been employed in Computer Vision for trajectory prediction from a single image \cite{DBLP:journals/corr/WalkerDGH16}  and frame prediction given a pair of frames \cite{}. 
Stochastic neural networks are networks where some of the activations are not deterministic but rather sampled from (often Gaussian)  distributions. Such normally distributed random variables are decoded after a series of convolutions and non-linear layers to highly multimodal distributions of the output space. 
In our work,  the means and variances of the Gaussian distributions  are deep non-linear transformations of the network input (the past visual history), that is, the stochastic layer is ``sandwiched" between deterministic encoder and decoder sub-networks, generalizing previous architectures of  \cite{DBLP:journals/corr/WalkerDGH16,NIPS2016_6552} which sampled from Gaussian unit variance noise. Once trained, sampling  the stochastic variables and decoding them  provides plausible samples of the future outcomes.

We present novel architectures and  training schemes for stochastic neural networks.   
For forecasting human body joint trajectories we introduce  \textit{conv-indexed  decoders}, depicted in Figure \ref{fig:Pnets}(b).   
%Body joint trajectories cannot be predicted using convolutional networks, since joints are present only on a handful of pixels, not at every pixel,
Previous works on body joint trajectory prediction  use fully connected layers since joints are present only on a handful of pixels, not at every pixel \cite{DBLP:journals/corr/WalkerDGH16}. This limits  generalization performance as each trajectory depends on the whole body configuration.  We instead use fully convolutional networks and index into the final convolutional feature map using the body joint pixel coordinates  -that are assumed known for the forecasting task. We thus predict body trajectories with a set of linear layers, one per body joint, each conditioned on a different feature embedding, extracted from the corresponding pixel location of the deconvolutional map.  
%We use one final linear transformation per body joint whose input feature vector is collected from the corresponding body joint location of the convolutional feature map. 
We empirically show that the proposed "as-convolutional-as possible" architecture outperforms by a margin fully connected alternatives \cite{DBLP:journals/corr/WalkerDGH16}.  Second, for frame prediction, we present \textit{stochastic dense spatial transformers}:  we compose the future video frame through prediction of a dense pixel motion field (optical flow) and differentiable backward warping that essentially re-arranges pixels of the input frame. Different samples from our model result in different future motion fields and corresponding frame warps. 

Training stochastic networks involves an intractable marginalization over the stochastic variables. We  present and compare  three  training schemes  that handle in different ways such intractable marginalization: a)  Straightforward   sampling for the prior. We simply collect samples from our Gaussian variables for each training example and maximize the empirical likelihood. b) Variational approximations, a.k.a. \textit{conditional variation autoencoders}  that sample from an approximate posterior distribution represented by a recognition model that has access to the output we want to predict. During training we minimize the Kullback–Leibler (KL) divergence between such informed posterior distribution and the prior  distribution provided by our generator model. c) $K$-best-loss, a loss we introduce in this work, which penalizes only \textit{the best  sample}  from a fixed ``prediction budget" for  each training example and training iteration. 
%Indeed, we empirically verify, that this is when K-best-loss outperfoms the alternatives. 



We evaluate the proposed architectures and training schemes on  three forecasting tasks:  (1) predicting motion trajectories (of pedestrians, vehicles, bicyclists etc.) from overhead cameras in the Stanford drone 
%campus
dataset~\cite{robicquet2016forecasting}, (2) predicting future body joint motion trajectories
%of human actors from 2D videos 
in the H3.6M dataset~\cite{h36m_pami},  and predicting future video frames ``in the wild''  using Freiburg-Berkeley Motion Segmentation~\cite{springerlink:10.1007/978-3-642-15555-0_21} and H3.6M datasets. We evaluate each training scheme under varying future  uncertainty: the longer the frame history we condition upon, the lesser the future uncertainty, the fewer the modes in the output distribution.  We show $K$-best-loss can better handle situations of \textit{high uncertainty}, with many \textit{equiprobable} outcomes, such as when predicting the future from a single image.  
%videos in the wild. 
%\TODO{JH - Is there a citation for the frame prediction in the wild data?}
%We perform a detailed comparison between the different training schemes and varying uncertainty and of our architectural contributions. 
We show extensive quantitative and qualitative results on paper and on our \href{https://sites.google.com/site/conditionalstochasticnets/}{online website}  
which confirm the validity of architectural innovations and facility of proposed training schemes.
%explaining the benefits of each.  





The closest works to ours are the work of Walker et al.  \cite{DBLP:journals/corr/WalkerDGH16} that predicts dense future trajectories from a single image and the work of Xue et al. \cite{NIPS2016_6552} that predicts a future frame given a pair of frames.   Both use stochastic units by sampling zero mean and unit variance Gaussian noise concatenated with the input feature maps and train using conditional variational autoencoders. Our work extends those in the following ways: a) proposes indexed convolutional decoders in place of fully connected decoders for trajectory forecasting and shows dramatic improvements, b)  proposes a novel $K$-best for training stochastic networks under extreme uncertainty, c) analyses the training  difficulties by comparing multiple training schemes under varying uncertainty, d) proposes a simpler architecture than \cite{NIPS2016_6552} based on optical flow warping for frame prediction and e) applies stochastic networks in diverse tasks and datasets.






\begin{figure}[t!]
\begin{center}
%\includegraphics[width=0.45\textwidth]{figs/Pnets2.pdf}
\includegraphics[width=0.45\textwidth]{figs/Pnets_latest.pdf}
\end{center}
\caption{\textbf{Conditional stochastic networks} for object trajectory forecasting (a), body joint trajectory forecasting (b) and video forecasting (c). Encoder,  stochastic and decoder subnetworks are depicted in green, gray and orange, respectively. 
\textit{(a):} Visual glimpses are centered around the object of interest. Glimpses here depict overhead camera views. 
%Though not shown, these two tasks share similar architectures differing only on the depth of the fully connected decoder.
\textit{(b):}  \textit{Conv-indexed decoders}  select feature vectors from a deconvolution network based on pixel coordinates, and predict each body joint trajectory using a separate linear layer on top of the selected feature vector. 
%To handle the non-convolutional nature of body joint trajectories, after a deconvolutional subnetwork, we index into its final feature map using the body joint locations and predict trajectories with a final linear layer, one per joint. We empirically show such conv-indexed decoders greatly outperform fully connected decoders of previous works, e.g., \cite{DBLP:journals/corr/WalkerDGH16}. 
%Though not shown, these two tasks share similar architectures differing only on the depth of the fully connected decoder.
\textit{(c):} Samples of future dense motion fields (future optical flows) differentiably warp the current frame to generate samples of the future one.
}
%, and estimate the parameters of our model by maximizing  log likelihood. }
\label{fig:Pnets}
\end{figure}




==> MotionPrediction (4)/macro.tex <==
%trajectory
\newcommand{\PP}{\mathrm{P}}
%\newcommand{\ncodes}{\mathrm{ncodes}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\Hor}{\mathrm{h}}
\newcommand{\logit}{\beta}
\newcommand{\deform}{\boldsymbol{\delta}}
\newcommand{\iorac}{i_{oracle}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\ncodes}{d}
\newcommand{\nsamples}{\mathrm{K}}
\newcommand{\ESDlong}{Encoder-Stochastic-Decoder}
\newcommand{\ESD}{ESD}
\newcommand{\ESDs}{ESDs}
\newcommand{\xx}{x}
\newcommand{\yout}{y}
\newcommand{\NN}{N}
\newcommand{\yhat}{\hat{y}}
\newcommand{\KK}{K}
%\newcommand{\encoder}{g}
%\newcommand{\decoder}{f}
\newcommand{\trx}{\mathrm{x}}
\newcommand{\try}{\mathrm{y}}
\newcommand{\ea}{\textit{et al.}}
\newcommand{\trz}{\mathrm{z}}
\newcommand{\encoder}{\mathrm{E}}
\newcommand{\decoder}{\mathrm{D}}
\newcommand{\zz}{z}

\newcommand{\MW}{W_\mu}
\newcommand{\SW}{W_\sigma}
\newcommand{\Mb}{b_\mu}
\newcommand{\Sb}{b_\sigma}
\newcommand{\N}{N}
\newcommand{\Nf}{N^f}

%\DeclareMathOperator*{\argmin}{arg\,min}

==> MotionPrediction (4)/model_arxiv.tex <==

\section{Conditional Stochastic Networks }\label{sec:model}




Figure~\ref{fig:Pnets} depicts our three stochastic network models for the three tasks we consider: (1) object trajectory forecasting, (2) body joint trajectory forecasting and (3) video prediction.  Samples  from our models correspond to  plausible future motion  trajectories  of the object,  future body joint trajectories of a person or future frame optical flow fields, respectively, for the three tasks we consider. 
%Our models are deep generative  neural networks that models the distribution of future outcomes conditioned on a sequence of visual glimpses. 



%\paragraph{Object-centric prediction}
%For the tasks of object and body joint motion trajectory forecasting, the conditioning history is centered around the human subject whose joints we want to predict:   By \textit{attending} (centering the visual glimpse) around the object of whose motion we want to predict we provide much less variable input, which facilitates the task by a lot as shown in previous work \cite{fragkiadaki2015learning,DBLP:journals/corr/BattagliaPLRK16}, at the expense of an object detector. Further, the same forecasting model can be shared by all objects in the scene to predict their future trajectories. 
%Such object centric prediction idea has been shown to be valuable against frame centric prediction in a number of recent works \cite{fragkiadaki2015learning,DBLP:journals/corr/BattagliaPLRK16}. 



% and takes as input a direct sequence of video frames. 
\paragraph{Object-centric prediction}
For dense pixel motion prediction,  visual glimpse correspond to the whole video frame.
For the case of object and body joint  trajectory forecasting however,   visual glimpses are 
centered around the object of interest. 
Such object-centric glimpses  
%deals with low resolution issues in case of  large image inputs and
%has been shown to have 
%a built-in translation invariance that helps to 
have been shown to generalize better to novel environments~\cite{fragkiadaki2015learning, DBLP:journals/corr/BattagliaPLRK16}, as they provide translation invariance. Further, the same forecasting model can be shared by all objects in the scene to predict their future trajectories. 



Our model has three components: an encoder $\encoder$, a stochastic layer $\zz$, and a decoder $\decoder$.  
The encoder is a deep convolutional neural network that takes as input a short sequence of visual glimpses $\xx$ and  computes a  feature hierarchy. The  stochastic layer is a $\ncodes$-dimensional  random variable $\zz$ drawn from a fully factored Gaussian distribution, whose means and standard deviations are parametrized by the top layer activations of the encoder $\encoder(\xx)$ through linear transformations $(\MW,\Mb)$ and $(\SW,\Sb)$:

\begin{align*}
\mu(x)&= \MW \cdot \encoder(\xx; \theta_\encoder) +\Mb, \\
\sigma(x)&= \log(\exp(\SW \cdot \encoder(\xx; \theta_{\encoder}) +\Sb)+1), \\
\zz &\sim \mathcal{N}(\mu, \mbox{diag}(\sigma)),
\end{align*}
For the standard deviations  we use a softplus nonlinearity to ensure positivity.  %\TODO{JH: Is $E^L$ different from $E$?}
The decoder $\decoder$ transforms samples of  $\zz$ (as well as encoder feature maps when skip-layers are present) to produce output $\yout$. While each of our stochastic variables $\zz$ follow a (unimodal) Gaussian distribution, 
the  distribution of $\yout$ can in general be highly multimodal as
shown qualitatively in Figure~\ref{fig:alahiqual} since Gaussian samples go through multiple non-linear layers. 
%.\TODO{fig:bodyjoints is missing?}

%Under standard maximum likelihood, conditioned on an input image sequence $\xx$, our model assumes that future motions  $\yout$ are normally distributed  with means that depend on the decoded random variables:
%\begin{align*}
%\yout &= ~ \mathcal{N}(\decoder(\zz \E(x;\theta)); \theta),\epsilon I), \, \epsilon \sim %\mathcal{N} (0,1), 
%\end{align*}
%\Jon{something wrong with the epsilon?}
%Notice that while we parametrize

The advantage of using a normal distribution for stochastic units is that back-propagation through the stochastic layer can be performed 
efficiently via the so-called \emph{reparametrization trick}~\cite{kingma2013auto,rezende2014stochastic}, where $\hat{\zz}$ denotes stochastic samples: 
 %\begin{equation}
 \begin{align}
 %\mu&= A_1 \cdot \encoder(\xx; \theta) +b_1, \\
%\sigma &= A_2 \cdot \encoder(\xx; \theta) +b_2, \\
%\mu, \sigma &= \encoder(\xx; \theta), \\
\hat{\zz} &=\mu(x)+ \epsilon' \cdot \sigma(x), \;\epsilon' \sim \mathcal{N} (0,I), \nonumber
\end{align}
%\end{equation}
%
%how we sample
 Given a visual glimpse sequence $x$, we obtain samples of future outcomes $\yhat $   by sampling our stochastic variables $\zz$:
 \begin{align*}
 %\mu&= A_1 \cdot \encoder(\xx; \theta) +b_1, \\
%\sigma &= A_2 \cdot \encoder(\xx; \theta) +b_2, \\
%\mu, \sigma &= \encoder(\xx; \theta), \\
\hat{\zz} &=\mu(x)+ \epsilon' \cdot \sigma(x), \;\epsilon' \sim \mathcal{N} (0,I), \\
\yhat &= \decoder(\hat{\zz}; \encoder(\xx; \theta_\encoder) ; \theta_\decoder),
\end{align*}
%\TODO{JH: do you mean to have yhathat in the above eqn?
%Also it's good if we write $\mu(x)$, $\sigma(x)$ to remind
%the reader of the dependencies.
%}
%
We train our model using maximum likelihood. 
We employ the standard assumption that ground-truth future outcomes $\yout$ are normally distributed  with means that depend on the output of our model. Let $\theta$  denote the weights of our stockastic network model, then we have:
\begin{align}
\yout &\sim \mathcal{N}(\decoder(\zz;\encoder(x;\theta_\encoder); \theta_\decoder),\nu  I). 
\end{align}
and maximize the marginal log likelihood $\mathcal{L}$ of the 
observed future outcomes conditioned on the input visual glimpses, as previous works:
\begin{small}
\begin{align}
&\mathcal{L}(\theta) \equiv \frac{1}{\N} \sum_{i=1}^\N \log  P(\yout^{(i)}) \equiv 
\frac{1}{\N} \sum_{i=1}^\N \log \int_{\zz^{(i)}} P(\yout^{(i)}, \zz^{(i)} | \xx^{(i)}) d\zz^{(i)} \nonumber \\
&\equiv   \frac{1}{\N} \sum_{i=1}^\N \log \int_{\zz^{(i)}} P(\yout^{(i)}, | \xx^{(i)},\zz^{(i)}) P(\zz^{(i)}|\xx^{(i)}) d\zz^{(i)} \label{eqn:marginalization2}
\end{align}
\end{small}
The marginalization across latent variables in Eq. \ref{eqn:marginalization2} is intractable. 
We will use the following three approximations: (1) a sample approximation to the marginal log likelihood by sampling from the prior (MCML), (2) variational approximations (VA) and (3) $K$-best-sample loss, as detailed below.

%\TODO{RS - you don't need the vspace{-2mm} if you don't accidentally start a new paragraph with a blank line after a block of math. A \% at the start of the line will also ensure this.}

\paragraph{Sampling from the prior (MCML)}
We maximize an approximation to the marginal log likelihood $\mathcal{L}$  using a set of $\nsamples$ samples for each of our $\N$ training examples: 
%\Jon{can we say this better?also! y is both a variable and the observed value!}
%Specifically, if we assume that the observed ground-truth displacements follow
%$\yhat = \yout+\epsilon$ where $\epsilon\sim \mathcal{N}(0, \nu)$ represents zero-mean gaussian noise, then we have:\vspace{-2mm}

\begin{small}
\begin{align}
&\mathcal{L}^{MCML}(\theta) \equiv   \frac{1}{\N} \sum_{i=1}^\N \log \sum^\nsamples_{\substack{j=1 \\ \hat{\zz}^{(i,j)} \sim P(\zz|\xx^{(i)})}} P(\yout^{(i)}| \hat{\zz}^{(i,j)}, \xx^{(i)}),\label{eqn:stochastic1} \\
    &=  \frac{1}{\N} \sum_{i=1}^\N \log \sum_{j=1}^\nsamples \exp\left( -\frac{\|\yhat^{(i,j)} - \yout^{(i)} \|^2}{2 \nu}\right) \label{eqn:logsumexp} 
\end{align}
\end{small}
\begin{comment}
\begin{small}
\begin{align}
&\mathcal{L}^{MCML}(\theta) \equiv  \frac{1}{\N} \sum_{i=1}^\N \log \int_{\zz^{(i)}} P(\yhat^{(i)}, \zz^{(i)} | \xx^{(i)}) d\zz^{(i)} \\
&\equiv   \frac{1}{\N} \sum_{i=1}^\N \log \int_{\zz^{(i)}} P(\yout^{(i)}, | \xx^{(i)},\zz^{(i)}) P(\zz^{(i)}|\xx^{(i)}) d\zz^{(i)}, \label{eqn:marginalization2}\\
    &\approx  \frac{1}{\N} \sum_{i=1}^\N \log \sum_{\substack{j=1 \cdots \nsamples \\ \zz^{(i,j)} \sim P(\zz|\xx^{(i)})}} P(\yout^{(i)}| \zz^{(i,j)}, \xx^{(i)}),\label{eqn:stochastic2} \\
    &=  \frac{1}{\N} \sum_{i=1}^\N \log \sum_{j=1}^\nsamples \exp\left( -\frac{\|\yhat^{(i,j)} - \yout^{(i)} \|^2}{2 \nu}\right) \label{eqn:logsumexp} 
\end{align}
\end{small}
\end{comment}
%\\
%    &= \max_\theta \frac{1}{\N} \sum_{i=1}^\N 
%    \left(-\frac{d^{(i)}}{2\nu}\right) +
%    \log \sum_{j=1}^\nsamples \exp\left( \frac{d^{(i)} - \|\yhat^{(i,j)} - \yout^{(i)} \|^2}{2 \nu}\right) \label{eqn:logsumexptrick} , \\
%    & d^{(i)} = \min_{j=1\cdots \nsamples} \| \yout^{(i)} - \yhat^{(i,j)} \|^2
%\vspace{-2mm}
%    &\approx \min_\theta \frac{1}{\N} \sum_{i=1}^m \min_{j=1}^\nsamples || \yhat^{(i)} - \yout^{(i,j)} ||^2.
%In the above, we have replaced Equation~\ref{eqn:marginalization2} with a sample approximation (Equation~\ref{eqn:stochastic}) over $\nsamples$ samples. 
%Further, in  Equation~\ref{eqn:exp}, we assume that the left hand term inside the exponent  dominates the right hand term.
We use $\nsamples=15$ samples for each training example.
%\TODO{JH: probably can drop the $\max_\theta$ in the above eqs 
%as well as below to 
%use less horizontal space.  Also I'm not sure I understand why 
%$d^{(i)}$ was introduced --- for numerical stability?  (If so, I'd
%probably just remove it)}
%In the last line, we
%view the log-sum-exp function as a smooth approximation to the max function (which becomes the min function after negation).



\begin{figure}[h!]
\begin{center}
%\includegraphics[width=0.45\textwidth]{figs/Q.pdf}
%\includegraphics[width=0.45\textwidth]{figs/Qnets.pdf}
\includegraphics[width=0.45\textwidth]{figs/Qnets_latest.pdf}
\end{center}
\caption{
\textbf{Recognition networks $Q$} for the tasks of body joint prediction and video prediction. The output $\yout$ is supplied as input to the model to provide an informative distribution over stochastic $\zz$ codes which our generator network $P$ tries to approximate.
}
\label{fig:Q}
\end{figure}

\paragraph{Variational approximation (VA)}
With a stochastic encoder and multimodal predictions, the likelihood of our model is sensitive to the sampling of the stochastic codes, which means, we would require a \textit{large amount of samples} to provide a good approximation to the marginal likelihood, which is the disadvantage of using MCML.  Another alternative is to do importance sampling in the stochastic codes, by taking into account the likelihood of each one.  
Returning to Equation~\ref{eqn:marginalization2} from the previous section, but doing importance sampling over our stochastic codes, our loss takes the form:
%\TODO{RS - Need alternative to this split + spanning double-column equation block. Putting in a figure* is one idea or defining additional terms and squeezing to one column. As is, it will confuse/annoy reviewers.}
{\small
\begin{align}
& \mathcal{L}(\theta) =
\frac{1}{\N} \sum_{i=1}^\N \log \int_{\zz^{(i)}} P(\yout^{(i)}, | \xx^{(i)},\zz^{(i)}) \nonumber \\
&\qquad \times \frac{P(\zz^{(i)}|\xx^{(i)})}{Q(\zz^{(i)} | \xx^{(i)} \yout^{(i)})}
Q(\zz^{(i)} | \xx^{(i)} \yout^{(i)}) d\zz^{(i)}, \label{eqn:mliw} \\
&\geq 
\mathcal{L}^{VA}(\theta) =
\frac{1}{\N} \sum_{i=1}^\N  \int_{\zz^{(i)}} 
Q(\zz^{(i)} | \xx^{(i)} \yout^{(i)}) d\zz^{(i)} \nonumber \\
& \qquad \times \log
P(\yout^{(i)}, | \xx^{(i)},\zz^{(i)})
\frac{P(\zz^{(i)}|\xx^{(i)})}{Q(\zz^{(i)} | \xx^{(i)} \yout^{(i)})} , \label{eqn:vaelower} \\
&= \frac{1}{\N} \sum_{i=1}^\N 
\mathbb{E}_{\zz\sim Q(\zz^{(i)} | \xx^{(i)} \yout^{(i)})} 
\left[ \log P(\yout^{(i)}, | \xx^{(i)},\zz^{(i)})\right] \nonumber \\
& \qquad - \textrm{D}_{\textrm{KL}} \left( Q(\zz^{(i)} | \xx^{(i)} \yout^{(i)}) \mid \mid P(\zz^{(i)} | \xx^{(i)}) \right), \label{eqn:vaeobj}
\end{align}\\
}
Equation~\ref{eqn:vaelower} is a lower bound of the importance 
weighted maximum likelihood objective (Equation~\ref{eqn:mliw}),
formed by taking the log of an expectation as the expectation of a log
using Jensen's inequality.
This requires creating a new approximation ($Q$) to the true posterior.  Here $Q$ attempts to give us
the best $\zz$ that can create a particular path $\yout$. 
In our final objective in Equation~\ref{eqn:vaeobj} we see that this
takes the form of a variational autoencoder style objective, as first noted in \cite{NIPS2015_5775}; since our $Q$ network further conditions on input $x$ (rather than just output $y$), it is called \textit{conditional} variational autoencoder.    
In the term on the left, we are just forming
maximum likelihood predictions, but using codes from our recognition network $Q$ (we found it sufficient to use only one sample per training example and iteration) instead of our generator, while the term on the right forces the distribution of the stochastic codes of our  recognition  network $Q$  and our generator to be close (in KL divergence terms).  
The architecture of our recognition networks for the tasks we consider are illustrated in Figure \ref{fig:Q}. At test time, of course only the generator model is used.

%\TODO{JH: Is $L^{VAE}$ really the best name?  This is a variational
%lower bound, but not an autoencoder (inputs are different
%from outputs).  Maybe just $L^{var}$?  Or are we viewing it as
%an autoencoder of $y$? that's conditioned on $x$?  Is this related
%to Honglak's CVAE papers?  Also, how is $Q$ parameterized in practice here?}





\paragraph{$K$-best-sample-loss (MCbest)}
We introduce $K$-best-sample-loss $\mathcal{L}^{best-sample}(\theta)$ that takes into account only the best sample within a budget of $\nsamples$ predictions, for each training example: 
\begin{small}
\begin{align}
& \mathcal{L}^{best-sample}(\theta) \equiv   \frac{1}{\N} \sum_{i=1}^\N \max_{\substack{j=1 \cdots \nsamples \\ \hat{\zz}^{(i,j)} \sim P(\zz|\xx^{(i)})}} P(\yout^{(i)}| \hat{\zz}^{(i,j)}, \xx^{(i)}),\label{eqn:stochastic} \\
    &\equiv  \frac{1}{\N} \sum_{i=1}^\N 
    \min_{j=1\cdots \nsamples} \| \yout^{(i)} - \yhat^{(i,j)} \|^2 
    \label{eqn:bestsample}
\end{align}%\vspace{-2mm}
\end{small}
%
Intuitively, for each training example during training, our model makes $\nsamples$ guesses (i.e. draws $\nsamples$ samples) about  the future outcome, not all of which have to be ``correct'' --- we only penalize the best guess made by the model for its deviation from ground-truth.  This approach consequently
encourages our model to ``cover its bases’’ by making diversified predictions. 

%Convex losses cannot cope with one-to-many mappings. 
%Regression-to-the-mean is a common failure mode in highly multimodal prediction problems which our model addresses.   For example, suppose there are two equally good (but distinct)
%trajectories that an agent can take;
%if our model can only make a single prediction and it is penalized by a convex loss (such as $L_2$), then the best thing for the model to do is to predict a convex combination between the two most likely trajectories (which itself might even be physically infeasible due to some obstacle).  Instead, our best-sample loss function encourages the model to properly predict both trajectories rather than to return a convex combination. Our experiments validate the superiority of this loss over maximum likelihood or variational approximation. 







==> MotionPrediction (4)/related.tex <==
\section{Related Work}

\paragraph{Multimodality in forecasting}
Handling multimodality in prediction is a notoriously difficult problem \cite{Theis2016a}. Models that minimize standard regression losses  perform poorly as they tend to regress towards a mean (blurry) outcome \cite{DBLP:journals/corr/MathieuCL15}.  Models that combine regression and adversarial losses \cite{DBLP:journals/corr/MathieuCL15} suffer  less from regression to the mean, but \textit{latch onto one mode of the distribution and neglect the rest},  as noted in \cite{Theis2016a}. Classifiers that employ  softmax losses need to discretize potentially  high-dimensional output spaces, such as pixel motion fields, and suffer from the corresponding discretization errors. Mixture component networks \cite{DBLP:journals/corr/Graves13,tuske_icassp2015} parametrize a Gaussian Mixture Model (GMM) (mixture components weights, means and variances) where  each mixture represents a different outcome. They have been  used successfully for hand writing generation in \cite{DBLP:journals/corr/Graves13} to predict the next $(x,y)$ pen stroke coordinate, given the generated writing so far. However, it is hard to train many mixtures of high dimensional output spaces, and, as it has been observed, many components often remain un-trained, with one component dominating the rest \cite{Fragkiadaki_2015_ICCV}, unless careful mixture balancing is designed \cite{DBLP:journals/corr/ShazeerMMDLHD17}. 
%Many works use the output of the network output to parametrize a single Gaussian distribution, its mean and variance. Though not multimodal, the model can handle uncertainty around a single  mode  better than a deterministic model.

%\vspace{-3mm}
%\paragraph{Motion forecasting}
%Early works on motion forecasting rely on the output of an object detector or image pixel labeller, in order to detect objects, free space and obstacles (trees, benches, sidewalks, roads)~\cite{robicquet2016forecasting,alahi2014socially,trautman2013robot,pellegrini2009you,antonini2006discrete,yamaguchi2011you,leal2011everybody,kitani2012activity}. 
%Most of the aforementioned approaches explicitly 
%incorporate physical  constraints or social interactions. 
%amongst people through  models that operate on the output of an object detector or scene labeling algorithm~\cite{robicquet2016forecasting,alahi2014socially,trautman2013robot,pellegrini2009you,antonini2006discrete,yamaguchi2011you,leal2011everybody}.\TODO{ref} 
%The design of such models incorporates the biases of the engineer regarding what ought to be important for motion prediction as opposed to discovering it directly from the observed pixels. 

%Traditional low-order parametric motion predictive models, e.g., constant velocity models~\cite{pellegrini2009you}, 
%to Markovian dynamics such as hidden Markov models, 
%Kalman filters~\cite{kalman1961new} and variants~\cite{schlenoff2004hierarchical,madhavan2003moving,Brand:1997:CHM:794189.794420,Ghahramani:1997:FHM:274158.274165,Weng:2006:VOT:1223195.1223208,thrun2005probabilistic} operate  on the output of an object detector and they aim to temporally smooth the detector's output. Thus, they are unable to anticipate motion reversal or deviations from smooth motion, e.g., a ball bouncing off a wall. 

Many recent data driven approaches predict motion directly from image pixels. 
%appearance is taken into account directly for motion prediction.
In \cite{walker2014patch}, 
a large, nonparametric image patch vocabulary is built for patch motion regression. In \cite{DBLP:journals/corr/WalkerGH15}, dense  optical flow is predicted from a single image and the multimodality of motion is handled by considering a different softmax loss for every pixel. 
Work of \cite{fragkiadaki2015learning} predicts ball trajectories in synthetic ``billiard-like'' worlds directly from a sequence of visual glimpses using a regression loss. Work of \cite{Fragkiadaki_2015_ICCV} uses recurrent networks to predict a set of body joint heatmaps at a future frame. Such representation though cannot possibly group the heatmap peaks into coherent 2D pose proposals.  Work of \cite{nal-vpn-2016}  casts frame prediction as sequential conditional prediction, and samples from a categorical distribution of 255 pixel values at every pixel location,  conditioning at the past history and image generated so far. It is unclear  %how to generalize such models for trajectory motion prediction, as well as 
how to handle  the computational overhead of such models effectively.

%We compare against such a model in our experiments and show that  regression losses underperform models that explicitly account for future uncertainty in the real world. 
%The proposed model in this work is considerably lighter from a computational point of view.
%Important exceptions are the works of Walker $\ea$~\cite{walker2014patch,DBLP:journals/corr/WalkerGH15,} and \cite{} \TODO{ref}. 
%For video frame prediction, the work of \cite{nal-vpn-2016} learns a probability distribution over pixel colors at every location and a video frame is generated through spatio-temporal conditional sequential sampling. Our model predicts motions instead of pixel colors, and pixel appearance is generated via differentiable warping using spatial transformers, which has been also used in the deterministic video prediction models of  \cite{DBLP:journals/corr/ByravanF16,DBLP:journals/corr/PatrauceanHC15}.
  %In this case, sequential conditional sampling is required to ensure that the prediction in one spatial location or temporal slice is taken into account when sampling motion for a different place or time, as done in the recent static image generation work of \cite{DBLP:journals/corr/OordKK16}. 
  %In this work, we bypass such complications by staying in the continuous domain of pixel displacements and employing stochastic units deep into the network model.
  %of the image 
  
  
%In this work, we rely instead on large video datasets to discover those rules directly from data, as well as others,
%that a hand-designed approach could have overlooked, e.g.,  the existence of specific jay-walking zones where extra traffic signs are necessary or there are too obvious to list, a.k.a. ``visual common sense" \cite{DBLP:journals/corr/LinP15}. 

\paragraph{Stochastic neural networks.}
Stochastic variables have been used in a variety of settings in the deep learning literature
e.g., for generative modeling, regularization, reinforcement learning, etc.  A key issue is how to train networks with stochastic
variables.  Restricted Boltzmann machines (RBMs), for example~\cite{hinton2006fast} are typically trained using MCMC sampling.  REINFORCE learning rules  were introduced by Willliams~\cite{williams1992simple} in order to  compute sample approximations to gradients in reinforcement learning settings and have also been useful in learning hard attention mechanisms~\cite{mnih2014recurrent,xu2015show,yeung2015end}.
In recent years papers have also proposed stochastic units that can be trained using ordinary SGD, with Dropout~\cite{srivastava2014dropout} being a ubiquitous example.  Another example is the so-called \emph{reparametrization trick} proposed by \cite{kingma2013auto,rezende2014stochastic} 
for backpropagation through certain stochastic units
(e.g., Gaussian) that allow one to differentiate quantities of the form $\mathbb{E}[f(x)]$ where $x\sim P(x; \theta)$ with respect to distribution parameters $\theta$.
Schulman~\ea~\cite{schulman2015gradient} recently united the REINFORCE and reparameterization tricks to handle backpropagation on general ``stochastic computation graphs’’.



%\vspace{-3mm}
\paragraph{Motion prediction as Inverse Optimal Control (IOC)}
%One way to effectively handle multimodality of motion trajectories is via inverse optimal %control. 
%In particular, the 
Works of \cite{ziebart2009planning,kitani2012activity,huang2015approximate} 
%predict human motion by 
model pedestrians as rational agents that move in a way that optimizes a reward function dependent on image features, e.g., obstacles in the scene, and form a distribution over optimal future paths to follow. They train a reward function 
such that the resulting Markov Decision Process  best matches  observed human trajectories in expectation. 
Many times though our motions/behaviours are not goal oriented and their framework fails to account for those. In these cases,  learning the possible future outcomes directly from data is important, as noted also in \cite{ziebart2010modelingB}. However, to deal with much longer temporal horizons we do expect that combination of planning and learning to be beneficial. 
%Yet, their proposed representation effectively handles multimodality of motion trajectories.



%Works of \cite{DBLP:journals/corr/0001ZXFT16,DBLP:journals/corr/WalkerDGH16} are most close to ours and employ stochastic networks for future prediction using variational approximations of the marginal likelihood. Our \ESD model proposes a different parametrization of the stochastic units conditioning them on input  visual history features, as opposed to concatenating samples from fixed Gaussians (noise) with deterministic visual features of the history, as in \cite{DBLP:journals/corr/0001ZXFT16,DBLP:journals/corr/WalkerDGH16}. Our decoder in many cases solely considers the sampled outcomes. Further, we propose a novel $K$-best-sample loss that we show outperforms variational approximations and demonstrate our model on object trajectory prediction with quantitative evaluation as opposed to only pixel generation.

%\TODO{
%four works most closely related to us
%Miost closely related to our works are the recent models of \cite{}.
%++alahi
%Forecasting Social Navigation in Crowded Complex Scenes
%https://arxiv.org/pdf/1601.00998v1.pdf
%flexible social forces model
%drone dataset
%\cite{DBLP:journals/corr/RobicquetASADWS16}
%Knowledge Transfer for Scene-specific Motion
%Prediction
%5https://arxiv.org/pdf/1603.06987v2.pdf
%\cite{DBLP:journals/corr/BallanCAPS16}
%}


%Inference in our model is a simple feed-forward evaluation of a deep network, making it an attractive alternative to models with complicated sequential conditional discrete sampling \cite{DBLP:journals/corr/WalkerGH15,DBLP:journals/corr/OordKK16} or to generative models  with intractable inference procedures \cite{sht-rtrbm-08}. 




%Aside of computatinal complexity, we would expect that a coarse to fine prediction would be more 

